Polyjuice: Generating Counterfactuals for Explaining, Evaluating, and Improving Models

While counterfactual examples are useful for analysis and training of NLP models, current generation methods either rely on manual labor to create very few counterfactuals, or only instantiate limited types of perturbations such as paraphrases or word substitutions. We present Polyjuice, a general-purpose counterfactual generator that allows for control over perturbation types and locations, trained by finetuning GPT-2 on multiple datasets of paired sentences. We show that Polyjuice produces diverse sets of realistic counterfactuals, which in turn are useful in various distinct applications: improving training and evaluation on three different tasks (with around 70% less annotation effort than manual generation), augmenting state-of-the-art explanation techniques, and supporting systematic counterfactual error analysis by revealing behaviors easily missed by human experts.

==> backup/_model.tex <==

\begin{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Modeling through Text Generation}
\label{subsec:nlg}

We frame counterfactual generation as a text generation task using language models (LMs).
Large pre-trained LMs like GPT-2~\cite{radford2019language} are capable of generating \emph{fluent} text.
They also increase the semantic and syntactic \emph{diversity}, by allowing for non-trivial counterfactuals with more flexibility than word substitutions~\cite{garg2019counterfactual} and templates~\cite{ribeiro2018sear}. 




\paragraph{The text prompt format.}
As shown in Figure~\ref{fig:blank}A, the input prompt to \sysname starts with $x$ followed by a special token (Line 1), which ensures that $\xp$ are conditioned on, and \emph{close} to $x$, rather than arbitrary text.
The generation can also be conditioned on \emph{\tagstrs} (Line 2) encoding the type of change, and \texttt{BLANK} \emph{tokens} (Line 3) specifying where changes happen.
These two encodings help achieve control over $\relation{\xp}$, such that \sysname fills in the blanks sequentially according to the controls (Line 4).
Note that the control conditions are optional.
When we exclusively condition the generation on $x$ (Line 1), \sysname can generate Line 2--3 on its own by sampling the \tagstr and the location of blanks.
% Next, we detail how we finetune GPT-2 to insert such formats.


\paragraph{\emph{Closeness} and \emph{Controllability}: Using \tagstrs and infilling structures.}
To build the close mapping between $x$ and $\xp$, we finetune GPT-2 on paired sentences, and create various training prompts from each paired $(x, \xp)$.
To control where in $x$ the perturbation happens, we extend the Infilling by Language Modeling (ILM) framework~\cite{donahue2020enabling}, such that $\xp$ contains \texttt{[BLANK]} tokens where perturbations are to be applied (Figure~\ref{fig:blank}A, Line 3). 
To allow flexible blanking, we also vary the location of \texttt{[BLANK]}s according to the example's parse tree.
As shown in Figure~\ref{fig:blank}B, Lines 6--9, such flexible placement allows for perturbations of any length (additions and deletions) beyond single word substitutions.


Moreover, to control the type of perturbations, we design special \tagstrs~\cite{raffel2019exploring, Dathathri2020Plug}, \eg \ctrltag{negation} in Figure \ref{fig:blank}A, Line 2.
Inspired by prior work categorizing manually created counterfactuals~\cite{kaushik2019learning, gardner2020contrast}, we define 8 \tagstrshorts (Table~\ref{table:ctrltag}) that distinguish lexical, syntactic, and semantic perturbations.
We compute the primary \tagstrshort based on linguistic features such as part-of-speech tags or dependency trees, and verify through an ablation study in Appendix~\ref{appendix:ablation_control} that training \sysname with \tagstrs greatly improves the success rate when generating counterfactuals that have these properties by 8\%--64\%.

\paragraph{\emph{Diversity}: Combining multiple paired sentences.}
We rely on six existing datasets of paired sentences, each containing counterfactuals with a subset of the \tagstrs of interest (see Table~\ref{table:ctrltag}). 
To increase diversity, we additionally find naturally occurring pairs in non-paired datasets like SQAuD~\cite{rajpurkar-etal-2016-squad}, using heuristics on the editing distance. 
%We use the pairs as negative samples if the change is too extensive.
A combination of these datasets yields a model that can produce \emph{diverse} counterfactuals.

We form $657,144$ training prompts from $191,415$ sentence pairs. 
More training prompt details and \tagstrshort statistics are in Appendix~\ref{appendix:train_data}.
Similar to \citet{madaan2020generate}, we quantitatively compare \sysname generations with baseline models.
As Appendix~\ref{appendix:intrinsic} summarizes, \sysname generates $\xp$ that are closer to $x$ than a standard generative model~\cite{Dathathri2020Plug} (\ie with much smaller syntactic editing distance~\cite{zhang1989simple}), and more diverse than off-the-shelf masked models like RoBERTa~\cite{liu2019roberta} (quantified using self-BLEU~\cite{zhu2018texygen}).




\paragraph{\emph{Fluency}: Through post-hoc filtering.}
Certain combinations of \tagstrs and \texttt{BLANK}s cause \sysname to generate ungrammatical or nonsensical counterfactuals 40\% of the time.
Similar to \citep{morris2020textattack}, we score both $x$ and $\xp$ using non-finetuned GPT-2, and filter out $\xp$ if its log-probability (either on the full sentence or on the perturbed chunks) decreases more than 10 points relative to $x$.
Because our applications in \S\ref{sec:app_label}--\S\ref{sec:app_err_analysis} all involve human teammates double checking the generation from \sysname, we intentionally select this loose threshold to present more \emph{diverse} counterfactuals. 
As further illustrated in \S\ref{subsec:label_efficiency}, we verify through human evaluation that the filtering improves the portion of fluent generations to 70\%--80\%, which we deem reasonable for the human to further inspect.
If used in a purely automated setting (\eg adversarial training), we can use filters or other constraints~\cite{morris2020textattack} to improve fluency (and/or semantic equivalence), at the cost of diversity --- rarer and more surprising changes may be blocked even if they are fluent. 


%(though their other constraints may also be useful.)


%\paragraph{Using counterfactuals.}
%\sysname is general-purpose and task-agnostic, and generates a variety of counterfactuals given one $x$. The most natural way to use \sysname is to generate $\hat{\xset}$ without constraints, and then select the counterfactuals in  $\hat{\xset}$ according to what is most appropriate for the task at hand (we provide examples of selection strategies for labeling and explanations in \S\ref{sec:app_label} and \S\ref{sec:app_explain}). However, users can also make use of the various control mechanisms, \eg generating counterfactuals by perturbing only specific subtrees of interest (an example is given in \S\ref{subsec:gen_counterfactual_for_labeling}).


% As a general-purpose and task-agnostic model, our generator does not distinguish counterfactual applications.
% Rather, it (targetedly) generates a large amount of counterfactuals with different combinations of \tagstrs and blanks, and the generated $\hat{\xset}$ should be further selected or ranked based on the relationship $\relation{\xp}$.
% For example, we find adversarial examples with common filtering constraints (\eg sentence semantic similarity~\cite{morris2020textattack}).
% We demonstrate different selections in \S\ref{sec:app_label} and \S\ref{sec:app_explain}.


%pr["pr_sent"]<=10 and pr["pr_phrase"] <=10
%Perplexity is instantiating; Language modeling as an approximation because it measures real world distribution.


\end{comment}

==> sections/__use_explanation_backup.tex <==
\definecolor{cfwone}{HTML}{eef5fa}
\definecolor{cfwtwo}{HTML}{daeaf5}
\definecolor{cfwthree}{HTML}{b2d2e9}
\definecolor{cfwfour}{HTML}{8abbde}

\newcommand{\fwone}[1]{\colbox{cfwone}{#1}\xspace}
\newcommand{\fwtwo}[1]{\colbox{cfwtwo}{#1}\xspace}
\newcommand{\fwthree}[1]{\colbox{cfwthree}{#1}\xspace}
\newcommand{\fwfour}[1]{\colbox{cfwfour}{#1}\xspace}

\newcommand{\fexp}[2]{\texttt{[{\color{darkgray}{#1:#2}}]}\xspace}
\newcommand{\fexptag}[1]{\fexp{TAG}{#1}}
\newcommand{\fexpfrom}[1]{\fexp{FROM}{#1}}
\newcommand{\fexpto}[1]{\fexp{TO}{#1}}
\newcommand{\fexptemp}[1]{\fexp{TEMP}{#1}}


\section{Counterfactual Explanations}
\label{sec:app_explain}

%Such explanations have been elusive in NLP, despite evidence from social science research~\cite{miller} indicating that they may be more intuitive, or may complement feature attribution or attention maps. 
%Counterfactuals also naturally support model explanations, as ``explanations are sought in response to particular counterfactual cases or foils''~\cite{miller}.
%Popular feature importance attribution methods like SHAP~\cite{NIPS2017_7062} or LIME~\cite{Ribeiro2016WhySI} all retrieve token importance through masking, which can be viewed as a form of (incomplete) counterfactual.




% \subsection{Foils to Feature Attribution Explanations}
A popular way of explaining NLP models is to attribute importance weights to the input tokens, either using attention scores~\cite{wiegreffe2019attention} or by summarizing the model behavior on perturbed instances (\eg LIME~\cite{Ribeiro2016WhySI} and SHAP~\cite{NIPS2017_7062}).
Even if token scores really reflect their real importance (\citet{pruthi2020learning} provided counter-examples), they can be too abstract for users to really understand model behavior~\cite{miller}. For example, while the explanation in Figure~\ref{fig:explanation}A indicates that the token ``help'' in Q2 is not very important, it's hard for users to grasp what that means without concrete examples, such as the one in Figure~\ref{fig:explanation}B. 

\begin{figure}[t]
\centering
\includegraphics[trim={0 21cm 33cm 0cm},clip,width=1\columnwidth]{figures/explanation_v2.pdf}
\vspace{-15pt}
\caption{
(A) A \qqp instance where the model\footnotemark{} predicts ``duplicate'' ($=$) with 98.2\% confidence, as well as the SHAP weights for tokens in Q2.
%Counterfactual explanations complement SHAP with concrete, readable examples, \eg (C) depicts a surprising flipped prediction ($\neq)$ that was missed by SHAP.
Counterfactual explanations complement SHAP with concrete examples and surprising behaviors, \eg (C)
depicts an unexpected flipped prediction ($\neq)$, given the low SHAP weight of the perturbed token \swap{friend}{woman}.
}
\vspace{-10pt}
\label{fig:explanation}
\end{figure}

\footnotetext{From BERT \qqp model: \url{https://huggingface.co/textattack/bert-base-uncased-QQP}}


That said, directly presenting a large number of concrete counterfactuals would be overwhelming, and so feature attribution methods are still useful as high level summaries.
One way to improve the explanation is to combine them with interactions, showing multiple \sysname counterfactuals that perturb the same span on-demand, a technique we explore in the next section. 
%as the alternative of presenting a large number of concrete counterfactuals would be overwhelming. 
%One way to improve them is by making them interactive, showing multiple \sysname counterfactuals that perturb the same span on-demand, a technique we explore in the next section. 
Here, we propose a complementary improvement: displaying a judicious selection of \sysname counterfactuals in addition to importance weights (Details in Appendix~\ref{appendix:exp_rank}). 
Following \citet{miller}'s observation that people look for explanations that reveal \emph{unexpected} behavior, we select \emph{surprising} counterfactuals that violate the expectations set by the feature attributions.
This includes examples where the \emph{real} change in prediction is large even though importance scores are low (Figure~\ref{fig:explanation}C, where perturbing the trivial ``friend'' results in flipped model prediction), and examples where the change is small but importance scores are high (Figure~\ref{fig:explanation}D).
%
%TODO: Do we want to cut this line?
If used with popular packages such LIME or SHAP, this procedure can also highlight their limitations: 
these methods usually estimate weights by \emph{masking} words, which may not correspond to natural counterfactual cases involving \eg word substitutions.


% This procedure also has the advantage of highlighting limitations of perturbations based on masking, used by popular packages such as LIME~\cite{Ribeiro2016WhySI} and SHAP~\cite{NIPS2017_7062}.


% While helpful as summaries, token scores may not reflect their real importance to the model, a limitation well known for attention~\cite{pruthi2020learning} and inherent to perturbation-based methods relying exclusively on masking tokens, \eg ``friend'' has near-zero weight in Figure~\ref{fig:explanation}, even though \swap{friend}{woman} flips the prediction in \ref{fig:explanation}C (\swap{friend}{[MASK]} has no effect on the prediction).


% 	B. Problem 1: can lead to error if it's too abstract, provide an example where a non important feature really is not important, but should be. Cite social science: people like counterfactuals, people like foils, people like concrete (is this in social science? Lol)
% Problem 2: relies on masking or attention, may not correspond to natural counterfactual cases


% Counterfactuals are essential for interpretability, as people seek for explanations through contrastive cases or ``foils.''~\cite{miller}.
% Because a large set of counterfactuals can be overwhelming, current techniques use feature attributions to summarize various local perturbations (\eg SHAP~\cite{NIPS2017_7062} or LIME~\cite{Ribeiro2016WhySI}).

% However, the resulting overview faces two challenges.
% First, feature weights can be too abstract for people to fully grasp.
% Without \swap{help}{find} in Figure~\ref{fig:explanation}B, an analyst viewing Figure~\ref{fig:explanation}A can hardly notice that the BERT \qqp model incorrectly assigns \remove{help} as a trivial feature.
% % see above for the actual quote. Did I interpret it correctly?
% Indeed, \citet{miller} argued that it may be unreasonable to expect a lay-user to be able to interpret an attribution, and that concrete foils are more intuitive.
% Second, feature attribution methods estimate weights by \emph{masking} words, which may not correspond to natural counterfactual cases involving \eg word substitutions.
% The usually overlooked gap can mislead analysts to over-generalize their perceived model behaviors.


% To address such issues, we present \sysname counterfactuals in addition to feature attributions.
% Following \citet{miller}'s observations that abnormal factors are more salient, we select counterfactuals that \emph{violate expectation}.
% That is, for each $\xp$, we compute the deviation of its \emph{actual} change of prediction from the \emph{expected} change, given the weights of perturbed features.
% We select $\xp$ that displays large prediction change, when small changes are expected. 
% In Figure~\ref{fig:explanation}C, \swap{friend}{woman} changes the prediction from \emph{Duplicate} to \emph{Non-Duplicate}, even though ``friend'' has low weight; 
% Conversely, we also include those with small changes, when large changes are expected.
% In Figure~\ref{fig:explanation}D, changing the important \remove{in depression} still results in \emph{Duplicate}.
% Computational details are in Appendix~\ref{appendix:exp_rank}.

% \subsection{User Evaluation}
% \label{subsec:exp_user_study}

\newcommand{\cshap}{\emph{\sysname-surprise}\xspace}
\newcommand{\crandom}{\emph{\sysname-random}\xspace}
\newcommand{\chuman}{\emph{Expert}\xspace}

\paragraph{User evaluation.} We study the scenario where an expert has access to a model and local explanations, and evaluate the \emph{additional} benefit of showing counterfactuals, \ie whether they bring \emph{new} insights. 
We evaluate three ways of generating counterfactuals: (1) \crandom, a baseline where we show random \sysname{} counterfactuals, (2) \chuman, where two graduate students (non-participants) were given access to the model and instructed to create counterfactuals that are surprising given the associated SHAP scores, and (3) \cshap, which uses the selection procedure described in the previous paragraph.
%The authors manually checked that all counterfactuals were fluent and unambiguous.
% We aim to answer: does seeing counterfactuals bring new insights, or are counterfactuals redundant with manual analysis or explanations?

We recruited 13 participants (graduate students with experience in model explanation), and had them analyze the aforementioned \qqp model. In each round, users were shown an example, the model prediction, and a SHAP explanation, as in Figure~\ref{fig:explanation}A. Users were instructed to create up to $10$ counterfactuals in order to better understand model behavior around the example, for which model predictions were given (users created $6$ on average). 
Finally, users simulated what the model would do on six counterfactuals, two from each condition (in random order). Counterfactuals where users make mistakes are preferable, as displaying these would add information that users do not already have.

% \paragraph{Setup.}
% We recruited 13 graduate students with experience in model explanations, and asked them to simulate the predictions of the aforementioned \qqp model on counterfactuals for 20 rounds.
% Intuitively, if the users are mistaken during the simulations, showing them such counterfactuals would add new information.
% In each round, the participants were given a base example, model prediction on it, and the SHAP weights, displayed as in Figure~\ref{fig:explanation}A.
% They could also create up to 10 counterfactuals to query model behaviors (they used around 6 chances.)
% Participants then simulated model predictions on six counterfactuals, two from each of the following conditions.
% We concluded the study with surveys on their query and simulation strategies.

% \paragraph{Conditions.} 
% We compare three types of counterfactuals:
% (1) \cshap, the \sysname-generated, abnormal counterfactuals, selected to complement SHAP; 
% (2) \crandom, the randomly selected \sysname counterfactuals; 
% (3) \chuman, the human-generated counterfactuals, in which two graduate students (not participants) played with the model, and each created one $\xp$ where the prediction was counter-intuitive according to the SHAP score on $x$.
% This is similar to hiring someone else to ``break the analysis'' with surprising examples.
%The authors manually checked that all counterfactuals were fluent and unambiguous.
% All the counterfactuals were close to the original examples, both in terms of the syntactic tree edit distance (0.97 in \cshap, to 1.25 in \chuman) and Levenshtein distance (around 0.2 in all conditions).
% \wts{remove Levenshtein here or add it to intrinsic evaluation part. this is what's used in MiCE.}

% \begin{comment}
\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{figures/err_rate.pdf}
\vspace{-15pt}
\caption{
Simulation error rates on counterfactuals. Higher error rates are better, indicating counterfactuals that would add more information to users if displayed.
}
\vspace{-10pt}
\label{fig:err_rate}
\end{figure}
% \end{comment}

\paragraph{Results.}
Figure~\ref{fig:err_rate} presents the simulation error rates. 
We see that humans can simulate model behavior on \cshap counterfactuals only slightly better than random guessing ($45\%\pm6\%$), \ie these examples display model behavior that is surprising to users even after seeing explanations and creating their own counterfactuals. \chuman counterfactuals also had a high error rate, but at a much higher cost: generating these for just 20 original instances took 1.5--2 hours of expert labor.

While high error rates could be achieved with unrelated or nonsensical examples, all counterfactuals under evaluation were close to the original examples, when measured by syntatic tree edit distance (${\approx}1.0$) or Levenshtein distance (${\approx}0.2$), \cshap being the closest on both. An independent rater labeled $95\%$ of \cshap counterfactuals as ``likely written by a native speaker'', in contrast to $85\%$ for \chuman, indicating that experts sometimes resorted to ungrammatical or nonsensical sentences in order to find surprising behaviors.

% Have to decide if it's worth keeping this paragraph
Qualitatively, the study participants tended to create counterfactuals by perturbing the token with the highest weights (84\% of their creations perturbed tokens in the top 15\% quantile of weights), not gaining a real understanding of how the other tokens impact predictions. Participants also made a significant number of mistakes even for tokens they had inspected, \eg a participant perturbed the example in Figure~\ref{fig:explanation}A by replacing \swap{help}{play with}, which the model predicts as \emph{Non-Duplicate}. When faced with \swap{help}{find} in Figure~\ref{fig:explanation}, they incorrectly assumed the behavior would be the same.

These results indicate that \sysname{} counterfactuals complement feature attribution explanations by displaying information that users often miss, even after they have manually explored the model behavior \emph{beyond} explanations. Moreover, \sysname{} counterfactuals for this application were more surprising and fluent than \chuman, despite being computed automatically at no extra cost.

% All the counterfactuals were close to the original examples, both in terms of the syntactic tree edit distance (0.97 in \cshap, to 1.25 in \chuman) and Levenshtein distance (around 0.2 in all conditions).
% \wts{remove Levenshtein here or add it to intrinsic evaluation part. this is what's used in MiCE.}

% As a within-subject study, we compared the error rate of human simulations across the three conditions.
% Participants only did slightly better than random guess on \cshap cases, with error rate $e=45\%\pm6\%$.
% If presented, these counterfactuals should bring more insights than hiring an expert graduate student to create counterfactuals ($e=39\%\pm11\%$), and more effectively: each graduate student had to spend 1.5--2 hours to generate 20 ``abnormal'' counterfactuals. 
% \crandom cases can be easily simulated ($e=23\%\pm6\%$), indicating the importance of abnormal counterfactuals.

% Another graduate student rated the fluency of counterfactuals, and verified that the simulation failure was not due to nonsensical noise.
% Interestingly, the rater deemed more than 95\% counterfactuals to be likely written by native speakers in both \sysname conditions, but only 85\% for \chuman, indicating that humans wrote ungrammatical sentences in order to find puzzling behavior.

% Participants' manual analysis revealed that they mostly erred when they missed the inspection spot.
% They focused mostly on what SHAP explanations deemed important, and ignored what was unimportant --- 84\% of their querying counterfactuals perturbed the most important features in the instance.\footnote{Tokens with weights higher than the 85\% quantile of all the weights in the instance.}
% For example, they repeatedly perturbed ``depression'' in Figure~\ref{fig:explanation}A, and therefore had to guess when simulating Figure~\ref{fig:explanation}B.
% In their survey responses, 7 participants explicitly stated their focus on important features, confirming that feature attributions can lead to incomplete comprehension.

% There are also 24\% of the missed \cshap cases where participants only partially inspected the related pattern,\footnote{At least one of their queries perturbed the same spans as $\xp$, and query text overlaps with the $\xp$ for over 70\%.} and were misled by it --- ``followed similar examples I tried,'' as one subject articulated.
% They could not to imagine the model predicting \emph{Duplicate} on Figure~\ref{fig:explanation}B (\swap{help}{find}), when it predicted \emph{Non-Duplicate} on their query \exinline{How do I \swap{help}{play with}...?}
% The number dropped to $15\%$ for the \chuman condition, showing that \cshap found more bugs in spots that participants considered inspected.

% \subsection{Discussions}

% \sysname counterfactuals is preferable over hiring a second expert analyst: they help find more insights at lower annotation cost, with less ungrammatical changes, and help extend manual inspection more exhaustively.
% However, certain forms of explanation selection is necessary to overcome the obvious ones. 
% The abnormality is one useful criteria that aligns with humans' cognitive processes, but humans should also be able to drive the selection, and acquire concrete foils for any spans \emph{they} do not understand.
% For example, an analyst can \texttt{BLANK} ``friend'' in Q2 in Figure~\ref{fig:explanation}C, and observe the model's unstable behavior: it predicts \emph{Non-duplicate} when \remove{friend} is changed to \add{woman}, \add{professional}, but remains \emph{Duplicate} at \add{man}, \add{student}.
% We discuss the interactions in \S\ref{sec:err_analysis}.

% As \citet{miller} noted, individual users should require less explanation the more they interact with a system.
% The fact that \sysname can still complement users' mental models, even after they see the feature attributions and manually inspect the model, indicates that the gain can be more prominent when such explanation and model access is not available. 
% We envision that the abnormality selection can also help select standalone explanations, if the expectation is instead estimated without feature attribution explanations (\eg he distance in the latent space~\cite{reimers-2019-sentence-bert}).
% We defer the exploration to future work.


==> sections/app_examples.tex <==

\begin{table*}[bp]
\small
\centering
\begin{tabular}{p{0.95\linewidth}}
\toprule
\textbf{Additional examples} \\ 
\midrule
It sucked \add{me in}. \\
\midrule

For those who are intrigued by politics of the '70s , the film is every bit as \swap{fascinating}{flawed} as it is \swap{flawed}{intriguing}. \\
\midrule

So exaggerated and broad that it comes off as \swap{annoying}{engaging} rather than \swap{charming}{annoying}. \\
\midrule

The film \swap{delivers}{doesn't deliver} what it promises: A look at the ``wild ride'' that ensues when brash young men set out to conquer the online world with laptops, cell phones and sketchy business plans. \\
\midrule

It's a crime movie made by someone who obviously knows \swap{nothing}{much} about crime. \\
\midrule

\swap{Even with}{Despite} all its botches, Enigma offers \swap{all}{none of} the pleasure of a handsome and well-made entertainment .\\
\midrule

``Catch Me'' feels \add{almost} capable of charming the masses with star power, a pop-induced score and sentimental moments that have become a Spielberg trademark.\\
\midrule

A sentimental but entirely \swap{irresistible}{unentertaining} portrait of three aging sisters.\\
\midrule

This is a movie full of \swap{grace}{mistakes} and, ultimately, \add{no} hope.\\
\midrule

Its simplicity puts an exclamation point on the fact that this isn't something to be taken seriously, but it also \swap{wrecks any chance}{poses an opportunity} of the movie rising above similar fare.\\
\midrule


\swap{If}{Even if} the film \swap{fails to fulfill}{succeeds in fulfilling} its own ambitious goals , it \swap{nonetheless sustains}{fails to sustain} interest during the long build-up of expository material .\\

\bottomrule
\end{tabular}
\vspace{-5pt}
\caption{Additional examples for Sentiment Analysis.}
%\wts{Change all the examples to be on an identical sentence, not all different cases. And consider further annotate the tags based on whether they just do semantic change or also syntactic change.}}
\label{table:sst_example}
\vspace{-10pt}
\end{table*}


\begin{table*}[bp]
\small
\centering
\begin{tabular}{p{0.95\linewidth}}
\toprule
\textbf{Additional examples} \\ 
\midrule


\textbf{Q1}: Poor people are more generous than rich people. Why? \newline
\textbf{Q2}: Is it true \swap{poor}{rich} people are more generous than \swap{rich}{poor} people? \\
\textbf{Q2}: Is it true poor people \swap{are more generous}{give more to charities} than rich people? \\
\midrule

\textbf{Q1}: Are TripAdvisor reviews more reliable than Yelp reviews because of their review process \newline
\textbf{Q2}: Are TripAdvisor reviews \swap{more}{less} reliable than Yelp reviews? \newline
\textbf{Q2}: Are TripAdvisor reviews more \swap{reliable}{unreliable} than Yelp reviews? \newline
\textbf{Q2}: Are \swap{TripAdvisor}{Yelp} reviews more reliable than \swap{Yelp}{TripAdvisor} reviews? \\
\midrule

\textbf{Q1}: How do you describe a smell? \newline
\textbf{Q2}: How will you describe a smell \swap{to}{from} a person? \newline
\textbf{Q2}: How will you describe a \swap{sound}{smell} to a person? \\
\midrule

\textbf{Q1}: Why are most psychopaths males and not females? and are female psychopaths different from male psychopaths? \newline
\textbf{Q2}: Is there a difference between male \remove{and female} psychopaths? \newline
\textbf{Q2}: Is there a difference between male and female \remove{psychopaths}? \newline
\textbf{Q2}: \add{Why} is there a difference between male and female psychopaths? \\
\midrule

\textbf{Q1}: How can I loose 5kgs weight in a week without exercise? \newline
\textbf{Q2}: How can I lose weight \swap{without}{by} doing exercise? \newline
\textbf{Q2}: How can I lose weight \remove{without doing exercise}? \newline
\textbf{Q2}: \swap{How can I}{Why can't you} lose weight without doing exercise? \\

\bottomrule
\end{tabular}
\vspace{-5pt}
\caption{Additional examples for Duplicate Question Detection, with the Q1 intact and Q2 changed.}
%\wts{Change all the examples to be on an identical sentence, not all different cases. And consider further annotate the tags based on whether they just do semantic change or also syntactic change.}}
\label{table:qqp_example}
\vspace{-10pt}
\end{table*}


\begin{table*}[bp]
\small
\centering
\begin{tabular}{p{0.95\linewidth}}
\toprule
\textbf{Additional examples} \\ 
\midrule

\textbf{P: }A small child stands in front of short white table.\newline
\textbf{H: }A child \swap{near}{sitting on} a table.\\
\midrule


\textbf{P: }A child sticks his head through a hole to create a picture of his head being a flower blossom\newline
\textbf{H: }The child is poking his head \swap{through}{to see} something.\\
\midrule

\textbf{P: }A young woman is playing fool.\newline
\textbf{H: }The woman is \swap{old}{very young} and not playing any games.\\
\midrule

\textbf{P: }Metal supports make a repeating X shape along the wall of the station.\newline
\textbf{H: }The walls are stronger with \swap{metal}{wood} supports rather than \swap{wood}{metal fences}.\newline
\textbf{H: }The walls are \swap{stronger}{less sturdy} with metal supports rather than wood.\\
\midrule

\textbf{P: }Several gentlemen are speaking into a microphone and the man in the glasses appears to be saying something funny\newline
\textbf{H: }Somebody \swap{that is shown wears}{shows} glasses.\\

\bottomrule
\end{tabular}
\vspace{-5pt}
\caption{Additional examples for Natural Language Inference, with the \textbf{P}remise intact and \textbf{H}ypothesis changed.}
%\wts{Change all the examples to be on an identical sentence, not all different cases. And consider further annotate the tags based on whether they just do semantic change or also syntactic change.}}
\label{table:nli_example}
\vspace{-10pt}
\end{table*}


\section{Additional counterfactuals}
\label{appendix:example}
Here, we include some additional counterfactual for each classification task.


==> sections/app_survey.tex <==


\begin{table*}[t]
\small
\centering
\setlength{\tabcolsep}{3.5pt}
\begin{tabular}{@{}l p{0.77\linewidth}@{}}
\toprule
\textbf{Application} & \textbf{Strategies} \\ 
\midrule
Data augmentation & 
    Lexical~\cite{Wu2019ConditionalBC, Wei2019EDAED, Kumar2020DataAU}\newline
    Paraphrasing~\cite{iyyer2018adversarial} \newline
    Perturbation functions~\cite{ratner2017snorkel}
\\\midrule
Counterfactual data aug. & 
    Manual~\cite{kaushik2019learning}
    Lexical~\cite{garg2019counterfactual}
\\\midrule
Adversarial attack & 
    Lexical~\cite{alzantot2018generating, garg2020bae, li-etal-2020-bert-attack, morris2020textattack, tan2020s, jin2020bert, ebrahimi2017hotflip, Zhang2019GeneratingFA, Jia2019CertifiedRT} \newline
    Template~\cite{jiang2019avoiding}\newline
    Insert~\cite{Song2020UniversalAA}
\\\midrule
Contrast set & 
    Manual~\cite{gardner2020contrast} \newline
    Templates~\cite{li2020linguistically}
\\\midrule
Challenge sets  & 
    Lexical (heuristic)~\cite{kaushik2019learning, naik2018stress} \newline
    Paraphrasing~\cite{Kavumba2019WhenCP} \newline
    Templates~\cite{Geiger2019PosingFG, kaushik2019learning, nie2019analyzing, mccoy2019right}
\\\midrule
Model analysis & 
    Lexical~\cite{garg2019counterfactual}\newline
    Template~\cite{Goodwin2020ProbingLS}\newline
    Perturbation functions~\cite{wu2019errudite, bowman-etal-2015-large, checklist:acl20}\newline
    Controlled text generation~\cite{madaan2020generate}
\\\midrule
Explanations & 
    Lexical~\cite{hase2020evaluating, vig2020causal, kang2020counterfactual} \newline
    % probably also lexical
    Lexical (through masking)~\cite{ramon2019counterfactual, ribeiro2018anchors}\newline
    Language model~\cite{ross2020explaining}
\\
\bottomrule
\end{tabular}
\vspace{-5pt}

\caption{A short survey on counterfactual application papers, and their generation strategies.}
\label{table:perturb_application}
%\end{table*}
\vspace{-10pt}

\end{table*}
%\end{comment}

\section{Survey of Perturbation Applications}
\label{appendix:paper_survey}

Table~\ref{table:perturb_application} summarizes existing applications of the counterfactuals, with their generation strategies.

